Inspecting Interactions: Online News Media Synergies in Social Media

The rising popularity of social media has radically changed the way news content is propagated, including interactive attempts with new dimensions. To date, traditional news media such as newspapers, television and radio have already adapted their activities to the online news media by utilizing social media, blogs, websites etc. This paper provides some insight into the social media presence of worldwide popular news media outlets. Despite the fact that these large news media propagate content via social media environments to a large extent and very little is known about the news item producers, providers and consumers in the news media community in social media.To better understand these interactions, this work aims to analyze news items in two large social media, Twitter and Facebook. Towards that end, we collected all published posts on Twitter and Facebook from 48 news media to perform descriptive and predictive analyses using the dataset of 152K tweets and 80K Facebook posts. We explored a set of news media that originate content by themselves in social media, those who distribute their news items to other news media and those who consume news content from other news media and/or share replicas. We propose a predictive model to increase news media popularity among readers based on the number of posts, number of followers and number of interactions performed within the news media community. The results manifested that, news media should disperse their own content and they should publish first in social media in order to become a popular news media and receive more attractions to their news items from news readers.

==> 3_Related_work.tex <==

\section{Related Work}
\label{sec:related_work}


%\reza{we need a story here, by saying what is the trend in news media studies (not from data driven approaches), what are the key research questions, and how our study is fiting to the current research. why we are novel in our approach or findings by showing this is a novel study?}
This section presents the literature review by summarizing the analysis of the news media presence in social media.
Researchers have analyzed the evolution of news media in online platforms in terms of their features and content \cite{132}. Some studies recommended that news stories are break up into shorter sentences in online platforms. For instance, online news stories are 20\% to 70\% shorter than print news stories \cite{133} . %In contrast, researchers also have studied the content of online newspapers and shown that the online newspapers mirrored the content found in print newspapers \cite{134}. 
In recent years, besides the news contents published in online Websites, those content has been shared in social media platforms as well.
The GO-Gulf team \cite{110} found that in social media, many people share pictures, opinions, status updates, recommendations and importantly, almost 22\% of shared items are news related content. Farahbakhsh et al. \cite{111} shown that the media news and news Websites are the most common type of content shared in social media, more than other categories such as political, commentary, sports, movies etc.
Major aspect of sharing news on social media is that individuals who perceive news will find them (news-finds-me-effect) are less likely to interact with traditional news sources \cite{78} which further reinforces the proposition that social media is playing a major role in readers' day-today news consumption.

There is a rapidly growing literatures that were analyzed the news media content shared on social media mainly focused on Facebook and Twitter platforms.  
Some studies \cite{97},\cite{98} claimed that even though Facebook has more users than Twitter, the latter is more widely used as a source of news. In particular, Twitter has been identified as a source of breaking news \cite{103} \cite{82} \cite{100} \cite{79}.
Alice et al. \cite{97} examined the effectiveness of Facebook and Twitter as news platforms and they argued on the existence of a positive relationship among newspapers' Facebook, Twitter, Web, and print readerships. In addition, previous work has focused on understanding the implications of news organizations' adaption of social media platforms through online readership and online traffic generated by social media sites. Their evidence suggest that the news media adoption of social media is positively associated with an increase in their online readership \cite{138}.

To this end, while there were different perspectives in the previous work to analyze news content in social media a few of them have focused on classifying news agencies in terms of the content they published based upon content originality. As mentioned earlier, since news media tend to use social platforms to share their content, it is worthwhile to analyze which news media is becoming popular among users with regard to readers' interactions and also content interactions among news media.
Hence, the aim of this study is to analyze different news media content shared in social media in terms of news originality, in order to identify which social media news users are providing more fresh news content to readers and which of them are consuming content from others.




